The landscape of bounds for binary search trees

Binary search trees (BSTs) with rotations can adapt to various kinds of structure in search sequences, achieving amortized access times substantially better than the Theta(log n) worst-case guarantee. Classical examples of structural properties include static optimality, sequential access, working set, key-independent optimality, and dynamic finger, all of which are now known to be achieved by the two famous online BST algorithms (Splay and Greedy). (...) In this paper, we introduce novel properties that explain the efficiency of sequences not captured by any of the previously known properties, and which provide new barriers to the dynamic optimality conjecture. We also establish connections between various properties, old and new. For instance, we show the following. (i) A tight bound of O(n log d) on the cost of Greedy for d-decomposable sequences. The result builds on the recent lazy finger result of Iacono and Langerman (SODA 2016). On the other hand, we show that lazy finger alone cannot explain the efficiency of pattern avoiding sequences even in some of the simplest cases. (ii) A hierarchy of bounds using multiple lazy fingers, addressing a recent question of Iacono and Langerman. (iii) The optimality of the Move-to-root heuristic in the key-independent setting introduced by Iacono (Algorithmica 2005). (iv) A new tool that allows combining any finite number of sound structural properties. As an application, we show an upper bound on the cost of a class of sequences that all known properties fail to capture. (v) The equivalence between two families of BST properties. The observation on which this connection is based was known before - we make it explicit, and apply it to classical BST properties. (...)

==> deterministic.tex <==
\input papervorspann

\begin{document}

Let $w_1$, \ldots $w_n$ be a sequence of weights. We show how to construct a tree in which the depth of element $\ell$ is $O(\log w[1:\ell]/\min(w_1,w_\ell))$. 

For $i \ge 1$, let $j_i$ be minimal such that $w[1:j_i] \ge 2^i w_1$. Then $w[1:j_i - 1] < 2^i w_1$ and 
$w[j_{i-1} + 1 : j_i] \le 2^{i-1} w_1 + w_{j_i}$. 

Let $T_i$ be the following tree. The right child of the root is the element $j_i$. The left subtree is a tree in which element $\ell$ has depth $O(\log 2^{i-1} w_1/w_\ell)$. 

The entire tree has $w_1$ in the root and then a long right spine. The trees $T_i$ hang off the spine to the left. In this way the depth of the root of $T_i$ is $O(i)$. 

Consider now an element $\ell$ in $T_i$. Assume first that $\ell \not= j_i$. The depth is
\[ O\left(i + \log \frac{2^{i-1} w_1}{w_\ell}\right) = O\left(i + \log \frac{2^{i-1} w_1}{\min(w_1,w_\ell)}\right)= 
O\left(\log \frac{2^{i-1} w_1}{\min(w_1,w_\ell)}\right)= O\left(\frac{w[1:\ell]}{\min(w_1,w_\ell)}\right).\]

For $\ell = j_i$, the depth is 
\[ O\left(i\right) = O\left( \log \frac{2^i w_1}{w_1} \right) = O\left(\log \frac{w[1:j_i]}{\min(w_1,w_{j_i})}\right) .\]

\end{document}



==> ki_movetoroot.tex <==
\section{Equivalence of Working set and key independent move-to-root bounds}

In this section we define a new bound called key independent move-to-root and show that it is the same as working set.

By an ordering $\Pi$ we mean the sequence $\{\pi(i)\}_{1}^{n}$, where $\pi$ is a permutation on $[n]$. Each ordering corresponds to a unique permutation and vice-versa; we will only consider orderings in this section.

Let $\mathcal{T}$ be a binary tree which is not a search tree. The order of elements in $\mathcal{T}$ is defined by $\Pi$, i.e. in-order traversal sequence of $\mathcal{T}$ is $\Pi$.

When we access an element $x$ in $\mathcal{T}$, we just bring $x$ to the root and that is it. No relative height between another element is changed, and no other rotations are performed. 
The cost is the length of the path from root to $x$ in $\mathcal{T}$.

\newcommand{\T}{\mathcal{T}}

Let $S$ be an access sequence.
The Move-To-Root bound with respect to an ordering $\Pi$, denoted as $\text{MTR}_{\Pi}(S)$, is the total cost of moving elements $s_{i}$ one by one to the root, starting from a tree with ordering $\Pi$. The effect of $S$ on $\T$ is
readily characterized in geometric view. When we access an element $s$ at time $t$, we lift it to height $t$ and do nothing else. It is the new root. The root of the left subtree is the highest element among the elements preceding $s$ in $\Pi$. 




Let \kimtr(S) = $\mathbb{E}_{\Pi} [\text{MTR}_{\Pi}(S)]$ (expectation over random $\Pi$). Recall that the working set bound $\ws(S)$ of an access sequence $S$ equals $\sum_{i=1}^{m} \log |W_{i}|$, where $W_{i}$ (called the working set of element $s_{i}$) is the number of distinct elements accessed since the last access of $s_{i}$ (before time $i$), and $|.|$ denotes its size.

\begin{theorem} $\kimtr(S) = \Theta( \ws(S) )$.
\end{theorem}

\begin{proof}

Let the working set of $s_{i}$ at time $i$ be of size $k$, and the last access of $s_{i}$ before time $i$ be at time $i-k^{'}$, for some $k^{'} \geq k$. We claim that in expectation, the cost of accessing $s_{i}$ at time $i$ in move-to-root is $\Theta( \log k )$. This would imply that every access contributes the same (upto constant factor) cost and we would establish the claim.

Let the working set of $s_{i}$ at time $i$ be $\{a_{0},\cdots,a_{k}\}$, with $a_{0} =s_{i-k^{'}} = s_{i}$. 
Because we ``move to root'' for each access, the $a_{i}$s are the $k$ highest elements in the current tree at time $i$. So $\mathcal{T}^{'} = \{a_{0},\cdots,a_{k}\}$  is a connected subtree containing the root. The expected depth of $s_{i-k^{'}}=s_i$ is $\Theta( \log k)$ because $\mathcal{T}^{'}$ is a random binary tree (we have taken expectation over all orderings $\Pi$).
\end{proof}

\noindent \textbf{Remark:} Eig says: I am not sure if this is really a "better" bound. 
At least, it says that, if you have a BST algorithm A which is competitive to MTR algorithm in binary tree with random ordering, then A satisfies working set (which implies static optimality, static finger, and log(n)-amortized cost).
